Direct neutrino-mass measurement based on 259 days of KATRIN data

The fact that neutrinos carry a non-vanishing rest mass is evidence of physics beyond the Standard Model of elementary particles. Their absolute mass bears important relevance from particle physics to cosmology. In this work, we report on the search for the effective electron antineutrino mass with the KATRIN experiment. KATRIN performs precision spectroscopy of the tritium $\beta$-decay close to the kinematic endpoint. Based on the first five neutrino-mass measurement campaigns, we derive a best-fit value of $m_\nu^{2} = {-0.14^{+0.13}_{-0.15}}~\mathrm{eV^2}$, resulting in an upper limit of $m_\nu < {0.45}~\mathrm{eV}$ at 90 % confidence level. With six times the statistics of previous data sets, amounting to 36 million electrons collected in 259 measurement days, a substantial reduction of the background level and improved systematic uncertainties, this result tightens KATRIN's previous bound by a factor of almost two.

==> authors.tex <==
\author{ KATRIN Collaboration:  Max~Aker, $^{1}$  \and Dominic~Batzler, $^{1}$  \and Armen~Beglarian, $^{2}$  \and Jan~Behrens, $^{1}$  \and Justus~Beisenk\"{o}tter, $^{3}$  \and Matteo~Biassoni, $^{4}$  \and Benedikt~Bieringer, $^{3}$  \and Yanina~Biondi, $^{1}$  \and Fabian~Block, $^{1}$  \and Steffen~Bobien, $^{5}$  \and Matthias~B\"{o}ttcher, $^{3}$  \and Beate~Bornschein, $^{1}$  \and Lutz~Bornschein, $^{1}$  \and Tom~S.~Caldwell, $^{6}$ $^{7}$  \and Marco~Carminati, $^{8}$ $^{9}$  \and Auttakit~Chatrabhuti, $^{10}$  \and Suren~Chilingaryan, $^{2}$  \and Byron~A.~Daniel, $^{11}$  \and Karol~Debowski, $^{12}$  \and Martin~Descher, $^{13}$  \and Deseada~D\'{i}az~Barrero, $^{1}$  \and Peter~J.~Doe, $^{14}$  \and Otokar~Dragoun, $^{15}$  \and Guido~Drexlin, $^{13}$  \and Frank~Edzards, $^{16}$ $^{17}$  \and Klaus~Eitel, $^{1}$  \and Enrico~Ellinger, $^{12}$  \and Ralph~Engel, $^{1}$ $^{13}$  \and Sanshiro~Enomoto, $^{14}$  \and Arne~Felden, $^{1}$  \and Caroline~Fengler, $^{1}$  \and Carlo~Fiorini, $^{8}$ $^{9}$  \and Joseph~A.~Formaggio, $^{18}$  \and Christian~Forstner, $^{16}$ $^{17}$  \and Florian~M.~Fr\"{a}nkle, $^{1}$  \and Kevin~Gauda, $^{3}$  \and Andrew~S.~Gavin, $^{6}$ $^{7}$  \and Woosik~Gil, $^{1}$  \and Ferenc~Gl\"{u}ck, $^{1}$  \and Steffen~Grohmann, $^{19}$  \and Robin~Gr\"{o}ssle, $^{1}$  \and Rainer~Gumbsheimer, $^{1}$  \and Nathanael~Gutknecht, $^{13}$  \and Volker~Hannen, $^{3}$  \and Leonard~Hasselmann, $^{1}$  \and Norman~Hau{\ss}mann, $^{12}$  \and Klaus~Helbing, $^{12}$  \and Hanna~Henke, $^{1}$  \and Svenja~Heyns, $^{1}$  \and Stephanie~Hickford, $^{1}$  \and Roman~Hiller, $^{1}$  \and David~Hillesheimer, $^{1}$  \and Dominic~Hinz, $^{1}$  \and Thomas~H\"{o}hn, $^{1}$  \and Anton~Huber, $^{1}$  \and Alexander~Jansen, $^{1}$  \and Christian~Karl, $^{16}$  \and Jonas~Kellerer, $^{1}$  \and Khanchai~Khosonthongkee, $^{20}$  \and Matthias~Kleifges, $^{2}$  \and Manuel~Klein, $^{1}$  \and Joshua~Kohpei\ss, $^{1}$  \and Christoph~K\"{o}hler, $^{16}$ $^{17}$  \and Leonard~K\"{o}llenberger, $^{1}$  \and Andreas~Kopmann, $^{2}$  \and Neven~Kova\v{c}, $^{1}$  \and Alojz~Koval\'{i}k, $^{15}$  \and Holger~Krause, $^{1}$  \and Luisa~La~Cascio, $^{13}$  \and Thierry~Lasserre, $^{21}$  \and Joscha~Lauer, $^{1}$  \and Thanh-Long~Le, $^{1}$  \and Ond\v{r}ej~Lebeda, $^{15}$  \and Bjoern~Lehnert, $^{22}$  \and Gen~Li, $^{11}$  \and Alexey~Lokhov, $^{13}$  \and Moritz~Machatschek, $^{1}$  \and Martin~Mark, $^{1}$  \and Alexander~Marsteller, $^{1}$ $^{14}$  \and Eric~L.~Martin, $^{6}$ $^{7}$ $^{23}$  \and Christin~Melzer, $^{1}$  \and Susanne~Mertens, $^{16}$ $^{17}$  \and Shailaja~Mohanty, $^{1}$  \and Jalal~Mostafa, $^{2}$  \and Klaus~M\"{u}ller, $^{1}$  \and Andrea~Nava, $^{4}$ $^{24}$  \and Holger~Neumann, $^{5}$  \and Simon~Niemes, $^{1}$  \and Anthony~Onillon, $^{16}$ $^{17}$  \and Diana~S.~Parno, $^{11}$  \and Maura~Pavan, $^{4}$ $^{24}$  \and Udomsilp~Pinsook, $^{10}$  \and Alan~W.~P.~Poon, $^{22}$  \and Jose~Manuel~Lopez~Poyato, $^{25}$  \and Stefano~Pozzi, $^{4}$  \and Florian~Priester, $^{1}$  \and Jan~R\'{a}li\v{s}, $^{15}$  \and Shivani~Ramachandran, $^{12}$  \and R.~G.~Hamish~Robertson, $^{14}$  \and Caroline~Rodenbeck, $^{1}$ $^{3}$  \and Marco~R\"{o}llig, $^{1}$  \and Carsten~R\"{o}ttele, $^{1}$  \and Milos~Ry\v{s}av\'{y}, $^{15}$  \and Rudolf~Sack, $^{1}$  \and Alejandro~Saenz, $^{26}$  \and Richard~Salomon, $^{3}$  \and Peter~Sch\"{a}fer, $^{1}$  \and Magnus~Schl\"{o}sser, $^{1}$  \and Klaus~Schl\"{o}sser, $^{1}$  \and Lisa~Schl\"{u}ter, $^{17}$ $^{22}$  \and Sonja~Schneidewind, $^{3}$  \and Ulrich~Schnurr, $^{1}$  \and Michael~Schrank, $^{1}$  \and Jannis~Sch\"{u}rmann, $^{3}$ $^{26}$  \and Ann-Kathrin~Sch\"{u}tz, $^{22}$  \and Alessandro~Schwemmer, $^{16}$ $^{17}$  \and Adrian~Schwenck, $^{1}$  \and Michal~\v{S}ef\v{c}\'{i}k, $^{15}$  \and Daniel~Siegmann, $^{16}$ $^{17}$  \and Frank~Simon, $^{2}$  \and Felix~Spanier, $^{27}$  \and Daniela~Spreng, $^{16}$ $^{17}$  \and Warintorn~Sreethawong, $^{20}$  \and Markus~Steidl, $^{1}$  \and Jaroslav~\v{S}torek, $^{1}$  \and Xaver~Stribl, $^{16}$ $^{17}$  \and Michael~Sturm, $^{1}$  \and Narumon~Suwonjandee, $^{10}$  \and Nicholas~Tan~Jerome, $^{2}$  \and Helmut~H.~Telle, $^{25}$  \and Larisa~A.~Thorne, $^{28}$  \and Thomas~Th\"{u}mmler, $^{1}$  \and Simon~Tirolf, $^{1}$  \and Nikita~Titov, $^{29}$  \and Igor~Tkachev, $^{29}$  \and Korbinian~Urban, $^{16}$ $^{17}$  \and Kathrin~Valerius, $^{1}$  \and Drahoslav~V\'{e}nos, $^{15}$  \and Christian~Weinheimer, $^{3}$  \and Stefan~Welte, $^{1}$  \and J\"{u}rgen~Wendel, $^{1}$  \and Christoph~Wiesinger, $^{16}$ $^{17}$  \and John~F.~Wilkerson, $^{30}$ $^{6}$ $^{7}$  \and Joachim~Wolf, $^{13}$  \and Sascha~W\"{u}stling, $^{2}$  \and Johanna~Wydra, $^{1}$  \and Weiran~Xu, $^{18}$  \and Sergey~Zadorozhny, $^{29}$  \and Genrich~Zeller $^{1}$  \\
\\
\normalsize{$^{1}$Institute for Astroparticle Physics~(IAP), Karlsruhe Institute of Technology~(KIT), } \\ 
\normalsize{Hermann-von-Helmholtz-Platz 1, 76344 Eggenstein-Leopoldshafen, Germany} \and 
\normalsize{$^{2}$Institute for Data Processing and Electronics~(IPE), Karlsruhe Institute of Technology~(KIT), } \\ 
\normalsize{Hermann-von-Helmholtz-Platz 1, 76344 Eggenstein-Leopoldshafen, Germany} \and 
\normalsize{$^{3}$Institute for Nuclear Physics, University of M\"{u}nster, } \\ 
\normalsize{Wilhelm-Klemm-Str.~9, 48149 M\"{u}nster, Germany} \and 
\normalsize{$^{4}$Istituto Nazionale di Fisica Nucleare (INFN) -- Sezione di Milano-Bicocca, } \\ 
\normalsize{Piazza della Scienza 3, 20126 Milano, Italy} \and 
\normalsize{$^{5}$Institute for Technical Physics~(ITEP), Karlsruhe Institute of Technology~(KIT), } \\ 
\normalsize{Hermann-von-Helmholtz-Platz 1, 76344 Eggenstein-Leopoldshafen, Germany} \and 
\normalsize{$^{6}$Department of Physics and Astronomy, University of North Carolina, Chapel Hill, NC 27599, USA} \and 
\normalsize{$^{7}$Triangle Universities Nuclear Laboratory, Durham, NC 27708, USA} \and 
\normalsize{$^{8}$Politecnico di Milano, Dipartimento di Elettronica, Informazione e Bioingegneria, } \\ 
\normalsize{Piazza L. da Vinci 32, 20133 Milano, Italy} \and 
\normalsize{$^{9}$Istituto Nazionale di Fisica Nucleare (INFN) -- Sezione di Milano, Via Celoria 16, 20133 Milano, Italy} \and 
\normalsize{$^{10}$Department of Physics, Faculty of Science, Chulalongkorn University, Bangkok 10330, Thailand} \and 
\normalsize{$^{11}$Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213, USA} \and 
\normalsize{$^{12}$Department of Physics, Faculty of Mathematics and Natural Sciences, University of Wuppertal, } \\ 
\normalsize{Gau{\ss}str.~20, 42119 Wuppertal, Germany} \and 
\normalsize{$^{13}$Institute of Experimental Particle Physics~(ETP), Karlsruhe Institute of Technology~(KIT), } \\ 
\normalsize{Wolfgang-Gaede-Str.~1, 76131 Karlsruhe, Germany} \and 
\normalsize{$^{14}$Center for Experimental Nuclear Physics and Astrophysics, and Dept.~of Physics, } \\ 
\normalsize{University of Washington, Seattle, WA 98195, USA} \and 
\normalsize{$^{15}$Nuclear Physics Institute,  Czech Academy of Sciences, 25068 \v{R}e\v{z}, Czech Republic} \and 
\normalsize{$^{16}$Technical University of Munich, TUM School of Natural Sciences, Physics Department, } \\ 
\normalsize{James-Franck-Stra\ss e 1, 85748 Garching, Germany} \and 
\normalsize{$^{17}$Max Planck Institute for Physics, Boltzmannstr. 8, 85748 Garching, Germany} \and 
\normalsize{$^{18}$Laboratory for Nuclear Science, Massachusetts Institute of Technology, } \\ 
\normalsize{77 Massachusetts Ave, Cambridge, MA 02139, USA} \and 
\normalsize{$^{19}$Karlsruhe Institute of Technology (KIT), Institute for Technical Thermodynamics and Refrigeration, } \\ 
\normalsize{Engler-Bunte-Ring 21, 76131 Karlsruhe, Germany} \and 
\normalsize{$^{20}$School of Physics and Center of Excellence in High Energy Physics and Astrophysics, } \\ 
\normalsize{Suranaree University of Technology, Nakhon Ratchasima 30000, Thailand} \and 
\normalsize{$^{21}$IRFU (DPhP \& APC), CEA, Universit\'{e} Paris-Saclay, 91191 Gif-sur-Yvette, France } \and 
\normalsize{$^{22}$Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA} \and 
\normalsize{$^{23}$Current address: Department of Physics, Duke University, Durham, NC, 27708, USA} \and 
\normalsize{$^{24}$Dipartimento di Fisica, Universit\`{a} di Milano - Bicocca, Piazza della Scienza 3, 20126 Milano, Italy} \and 
\normalsize{$^{25}$Departamento de Qu\'{i}mica F\'{i}sica Aplicada, Universidad Autonoma de Madrid, } \\ 
\normalsize{Campus de Cantoblanco, 28049 Madrid, Spain} \and 
\normalsize{$^{26}$Institut f\"{u}r Physik, Humboldt-Universit\"{a}t zu Berlin, Newtonstr.~~15, 12489 Berlin, Germany} \and 
\normalsize{$^{27}$Institute for Theoretical Astrophysics, University of Heidelberg, } \\ 
\normalsize{Albert-Ueberle-Str.~2, 69120 Heidelberg, Germany} \and 
\normalsize{$^{28}$Institut f\"{u}r Physik, Johannes-Gutenberg-Universit\"{a}t Mainz, 55099 Mainz, Germany} \and 
\normalsize{$^{29}$Institute for Nuclear Research of Russian Academy of Sciences, } \\ 
\normalsize{60th October Anniversary Prospect 7a, 117312 Moscow, Russia\footnote{Institutional status in the KATRIN Collaboration has been suspended since February 24, 2022}} \and 
\normalsize{$^{30}$Also affiliated with Oak Ridge National Laboratory, Oak Ridge, TN 37831, USA} }
